Finite-Sample-Based Reachability for Safe Control with Gaussian Process Dynamics

Gaussian Process (GP) regression is shown to be effective for learning unknown dynamics, enabling efficient and safety-aware control strategies across diverse applications. However, existing GP-based model predictive control (GP-MPC) methods either rely on approximations, thus lacking guarantees, or are overly conservative, which limits their practical utility. To close this gap, we present a sampling-based framework that efficiently propagates the model's epistemic uncertainty while avoiding conservatism. We establish a novel sample complexity result that enables the construction of a reachable set using a finite number of dynamics functions sampled from the GP posterior. Building on this, we design a sampling-based GP-MPC scheme that is recursively feasible and guarantees closed-loop safety and stability with high probability. Finally, we showcase the effectiveness of our method on two numerical examples, highlighting accurate reachable set over-approximation and safe closed-loop performance.

==> extra/extra.tex <==
Applying the same control input and using the dynamics \ref{eq:system_dyn}

If we sample $\Tilde{N}$ dynamics then with probability $1-\delta$ there is at least one dynamic which is $\epsilon$ close.


\manish{Check we don't need dynamics close everywhere by only at the next prediction we need at least one should be epsilon close}
% \end{proof}




% \begin{theorem}[Probabilistic reachable set]
% For any control policy $\coninput(k)$,
%     \begin{align*}
%        Pr\{ \mathcal{R}_k(x_0, \dynGPtrue) \in \mathcal{R}_k(x_0, \mathcal{G}),~\forall k \in [\horizon] \} \geq 1- \delta  
%     \end{align*}
% \end{theorem}

Find a control input $\coninput$ such that $\mathcal{R}_k(x_0, \mathcal{G}), \pi_k \in \mathcal{Z}$.

\mypar{Objective} Find the \# samples $N$ such that $\exists \dynGP^i, i \in [N]: \| \dynGP^i - \dynGPtrue \|_{\infty} \leq \epsilon$ with probability at least $1-\delta$.

Consider a ball, 
\begin{align*}
    B_{\epsilon}(\mathbf{0}) = \{ f \in \mathbb{B}~|~\|f-\mathbf{0}\|_{\infty} \leq \epsilon \}
\end{align*}


\begin{lemma}[Cameron-Martin formula]
    If $\dynGPtrue \in \RKHS$, then for a set $B_{\epsilon}(\mathbf{0}) \subset \mathbb{B}$, where $\mathbb{B}$ is a Banach space equipped with some norm, e.g., infinity
    \begin{align*}
        P( \dynGP^i - \dynGPtrue \in B_{\epsilon}(\mathbf{0})) \geq e^{-\frac{1}{2}\|\dynGPtrue-\mu\|^2_{\RKHS}} P( \dynGP^i - \mu \in B_{\epsilon}(\mathbf{0})).
    \end{align*}
\end{lemma}

% \begin{proof}
%     In our case Banach space $\mathbb{B}$ is equipped with an infinity norm.
%     \begin{itemize}
%         \item For referring \cite[Lemma 5.2]{van2008reproducing} use $W = \dynGP^i - \mu$, \red{$h = \dynGPtrue - \mu$} and $C =  B_{\epsilon}(\mathbf{0})$.
%         \item $\dynGP^i - \mu$ and $-(\dynGP^i - \mu)$ are identically distributed since they are samples of GPs and centred around mean
%         \item $B_{\epsilon}(\mathbf{0}) = - B_{\epsilon}(\mathbf{0})$ since its a ball: $B_{\epsilon}(\mathbf{0}) = \{ f \in \mathbb{B}~|~\|f - \mathbf{0}\|_{\infty} \leq \epsilon\}$.
%         \item $\dynGPtrue \in \RKHS$ and $\mu \in \RKHS$ implies $\dynGPtrue -\mu \in \RKHS$, since it is a vector space
%     \end{itemize}
%     \begin{align*}
%         P( \dynGP^i - \dynGPtrue \in B_{\epsilon}(\mathbf{0})) &= P( \dynGP^i - \mu - (\dynGPtrue - \mu) \in B_{\epsilon}(\mathbf{0}))\\
%         &\geq e^{-\frac{1}{2}\|\dynGPtrue-\mu\|^2_{\RKHS}} P( \dynGP^i - \mu \in B_{\epsilon}(\mathbf{0})) \\
%         & =  e^{-\frac{1}{2}\|\dynGPtrue-\mu\|^2_{\RKHS}} e^{-\phi_{\mu}(\epsilon)} \\
%         &\geq %e^{-\frac{1}{2}(\|\dynGPtrue\|^2_\RKHS +  \|\mu\|^2_{\RKHS})} e^{-\phi_{\mu}(\epsilon)} = 
%         e^{-B} e^{-\phi_{\mu}(\epsilon)} = e^{-\left(B+\phi_{\mu}(\epsilon)\right)}
%     \end{align*}
% In the above, $P( \dynGP^i - \mu \in B_{\epsilon}(\mathbf{0})) = e^{-\phi_{\mu}(\epsilon)}$.  \manish{Cameron-Martin formula, shift of Gaussian measure}
% \end{proof}
% \manish{Not sure about the content around eqn 5.1 in \cite{van2008reproducing}} \\
Note the following:
\begin{align*}
    g(y) &= \sum_{i=1}^n \alpha_i k(y,x_i)   \\
    g(x) &= \left\langle g(\cdot), k(\cdot,x) \right\rangle_{\RKHS} = \left\langle \sum_{i=1}^n \alpha_i k(y,x_i), k(y,x) \right\rangle_{\RKHS} \\
         &= \sum_{i=1}^n \alpha_i k(x,x_i) = g(x)
\end{align*}
Hence (See \cite{steinwart2008support}, eq 4.8),
\begin{align*}
    |g(x)| &= |\langle g(\cdot), k(\cdot,x) \rangle_{\RKHS}| \leq \|g\|_{\RKHS} \|k(\cdot,x)\|_{\RKHS} =  \|g\|_{\RKHS} \langle k(\cdot,x), k(\cdot,x)\rangle_{\RKHS} = \|g\|_{\RKHS} k(x,x)^{1/2} \leq \|g\|_{\RKHS} k_{\infty}\\ 
\end{align*}



$P( \|\dynGP^i - \dynGPtrue\|_{\infty} \leq \epsilon' ) \geq P( \|\dynGP^i - \dynGPtrue\|_{\RKHS} \leq \epsilon'/k_{\infty}) \geq  e^{-(B + \phi_{\mu}(\epsilon))}$. (Use $\epsilon = \epsilon'/k_{\infty}$). 

In the following lemma: $P( \|\dynGP^i - \dynGPtrue\|_{\RKHS} \leq \epsilon) \geq 1 - \delta \implies P( \|\dynGP^i - \dynGPtrue\|_{\infty} \leq \epsilon') \geq 1 - \delta$ and $\phi_{\mu}(\epsilon) = -\log( P( \|\dynGP^i - \mu\|_{\RKHS} ) \leq \epsilon)$ 
 is in the RKHS norm.

\begin{lemma}
Derive sample complexity bound for infinite dimension case.
\end{lemma}
\begin{proof}
Number of samples bound: Let's say we need $N$ samples to guarantee least one of the samples is in the ball of radius $\epsilon$.



\end{proof}


\manish{Either use $\dynGPtrue - \mu \leq \beta \sigma$ or $\dynGPtrue - \mu \leq B$. For the former one, we may again need $\|\sigma\| \leq k(x,x) \leq 1$ or so.}

Bounds to follow:
After $k$ steps $|x_k - x^{tr}_k| \leq \epsilon L_g^k = \Tilde{\epsilon}$. Shrink your constraint set by $\Tilde{\epsilon}$.



\manish{
\begin{itemize}
    \item Is order type analysis fine or should we focus on constants as well? --- Constants are fine as well
    \item Support of samples is the closure of RKHS? With probability 1 the sample doesn't lie in the RKHS space? We can increase the space with some power and it works? Which norm does the Cameron-Martin hold with then? -- not a contradiction since we are finding a sample that is epsilon close in the infinity norm and don't care if sample is in the RKHS space
    \item Prior vs posterior vs online learning --- How does the bound vary? --- intuitively we only need to change the norm with the new RKHS space and then it should be fine as well ... since the posterior update is again a GP with new kernel and mean (does subtracting from posterior mean is again fine?). Andreas showed us the equation of how the RKHS norm grows with samples
\end{itemize} }









\begin{itemize}
    \item Sample complexity result. Let N be the smallest integer satisfying equation, then there exists at least one sample that lies in an epsilon ball around the true function with probability $1-\delta$.
    \item Solve the MPC problem with $\Tilde{N}$ and constraints tightened with $\epsilon' = \epsilon L^H$, then with probability $1-\delta$ problem is recursively feasible and satisfy the original constraints (without tightening).
    \item RTI argument -- if initialization is closed enough then solution is also good
\end{itemize}

Potential improvements from CDC version
\begin{itemize}
    \item Efficient solver by using fantasy updates? (can also do it in CDC)
    \item New simulations with epsilon tightening
    \item Any algorithmic changes? (keeping past L samples instead of just the last 1, already in CDC paper)
    \item 
\end{itemize}

sample complexity 

Probabilistic reachable sets

MPC
- closed loop

Numerical section: how we sample from GP
- remark closed loop guarantee decay

Simulation

Conclusion

new section on Method -- MPC result

open loop easy 

close loop guarantees will get worse with time or keep all the samples from the past --- can we use some ideas from stochastic MPC -- check the last input if the problem is not feasible



\begin{theorem}
Let \cref{assump:q_RKHS,assump:lipschitz_dyn,assum:safeset} hold. Pick an $\epsmpc > 0$ in Problem \eqref{eq:SafeGPMPCinf} and $\Tilde{N}$ be as defined in \cref{thm:sample_complexity} with $\epsdyn \coloneqq \epsmpc / L_H$. If Problem \eqref{eq:SafeGPMPCinf} is feasible at $\ki=0$, then with probability at least $1-\delta$, \eqref{eq:SafeGPMPCinf} is recursively feasible $\forall \ki \in \mathbb{N}$, and the constraints are satisfied, i.e., $(\state(\ki), \coninput(\ki)) \in \mathcal{Z}$ ~$\forall k\in\mathbb{N}$, for the closed-loop system resulting from Problem \eqref{eq:SafeGPMPCinf}.
\end{theorem}
\begin{proof}
% First, note that $\dynGP^{\mathrm{tr}} \in \dynSet$ with probability at least $1-\prob$ due to \cref{thm: beta}. 
To show recursive feasibility, we use a standard proof with a candidate solution~\cite{rawlingsModelPredictiveControl2020}: Denote the optimal input sequence at time $\ki$ as $\bm{\coninput}^\star = \{\coninput_0,\dots, \coninput_{\horizon-1}\}$. 
At time $\ki + 1$, we consider the candidate input sequence
\mbox{$\bm{\coninput}=\{\coninput_1,\dots, \coninput_{\horizon-1}, \coninput_{\mathrm{f}}\}$} where $u_{\mathrm{f}}$ ensures positive invariance of the terminal set constraint (\cref{assum:safeset}). 

Given Problem $\eqref{eq:SafeGPMPCinf}$ uses $\Tilde{N}$ samples, then with probability at least $1-\delta$, $\exists \n \leq \Tilde{N}: \|\dynGP^\n - \dynGPtrue \| \leq \epsdyn$. At time $\ki+1$, 
starting with $\|x_{0|\ki+1} - \state^\n_{0|\ki+1}\| \leq \Lipdyn \epsilon \implies \|x_{\horizon-1|\ki-1} - \state^\n_{\horizon-1|\ki-1}\| \leq \epsdyn L_{\horizon-1} \Lipdyn + \epsdyn = \epsmpc$ which is the tightening used in constraints (including terminal set) of Problem \eqref{eq:SafeGPMPCinf}. 
All the samples are initialized with $\state^\n_{0|\ki+1} = \lambda x(t)+(1-\lambda) x_{1|t-1}^\n, \lambda\in [0,1]$ which ensures that the old input sequence is still feasible for all the sampled dynamics.
Using \cref{assum:safeset}, there exists a control input $\coninput_{\mathrm{f}}$ that keeps all the trajectories in the terminal set $\mathcal{Z}_f \ominus B_{\epsmpc}(\mathbf{0})$. Hence, this input sequence is a feasible solution to Problem \eqref{eq:SafeGPMPCinf} and thus \eqref{eq:SafeGPMPCinf} is recursively feasible.

% \manish{Why starting at $x(\ki+1)$ and applying the same control sequence is still feasible?}

Constraint satisfaction guarantees follow directly from the feasibility of Problem \eqref{eq:SafeGPMPCinf} and constraint \eqref{eqn:state_input_constraint} for $i=0$. Note that the system always stays inside the probabilistic reachable set \cref{thm:PRS} (or the constrained tightening is same using the PRS) which guarantees safety with high probability. 
\end{proof}





% \author{Manish Prajapat, Johannes K\"ohler, Matteo Turchetta, Andreas Krause$^\dagger$, Melanie N. Zeilinger$^\dagger$ \thanks{\looseness -1 $\dagger$ Joint supervision. All authors are from ETH Zurich. [manishp, jkoehle, matteotu, krausea, mzeilinger]@ethz.ch. Manish Prajapat is supported by ETH AI center, Johannes K\"ohler and Matteo Turchetta by the Swiss National Science Foundation under NCCR Automation, grant agreement 51NF40 180545.}}

% \thanks[footnoteinfo]{$\dagger$ The work is jointly supervised by Melanie N. Zeilinger and Andreas Krause. 
% Manish Prajapat is supported by ETH AI center and Johannes K\"ohler by the Swiss National Science Foundation under NCCR Automation, grant agreement 51NF40 180545.}

% \author[ai_center,idsc,eth_cs]{Manish Prajapat}\ead{manishp@ai.ethz.ch},
% \author[idsc]{Johannes K\"ohler},
% \author[idsc]{Amon Lahr},    % Add the 
% \author[ai_center,idsc]{Melanie N. Zeilinger$^\dagger$},               % e-mail address 
% \author[ai_center,eth_cs]{Andreas Krause$^\dagger$}  % (ead) as shown

% \address[ai_center]{ETH AI Center, ETH Zurich, Switzerland}  % Please supply                               
% \address[idsc]{Institute for Dynamic Systems and Control, ETH Zurich, Switzerland}             % full addresses
% \address[eth_cs]{Department of Computer Science, ETH Zurich, Switzerland}

==> extra/lip_lyapunov_small_ball.tex <==
\newpage

\manish{The following lemma is not required due to \cref{lem:small_ball_comparison_prior_posterior_variance}. I will remove it later. Please directly see the next subsection.}
\begin{lemma} \label{lem:posterior_small_ball}
    For a posterior kernel $k_D$ defined by   \cref{eq:kernel_posterior_update} with a Matern prior $k$ and $\dynGP \sim \GP(\mu_D, k_D)$, there exists a constant C independent of $\epsilon$ such that,
    \begin{align}\label{eq:posterior_small_ball}
        -\log \probability{\|\dynGP - \mu_D \|_{\infty} \leq \epsilon) \leq C \left(\frac{1}{\epsilon}\right)^{d/\alpha}}.
    \end{align}
\end{lemma}
\begin{proof}
Let $U_k$ and $U_{k_D}$ be the unit balls of $\RKHS$ and $\RKHSdata$ respectively. Note that due to \cref{eq:rkhsnorm_equivalence}, we get $\RKHS = \RKHSdata$ however RKHS norm of the posterior kernel is higher which implies $U_{k_D} \subseteq U_k$.

Consider metric entropy $H(U_k, \epsilon) = \log N(U_k,\epsilon)$ of unit ball $U_k$, where $N(U_k,\epsilon)$ is minimum covering number (covering $U_k$ with balls of radius $\epsilon$ in infinity norm). Analogously we can define it for $U_{k_D}$ as $H(U_{k_D}, \epsilon)$.
\begin{align}
    U_{k_D} \subseteq U_k \implies H(U_{k_D}, \epsilon) \leq H(U_k, \epsilon) \label{eq:covering_relation}
\end{align}
Thus, the covering number for the prior also bounds that of the posterior kernel. Using \cite[Theorem 1.2]{li1999approximation} which characterises small ball probability $\phi(\epsilon)$ in terms of metric entropy we get the required bound, i.e., \cref{eq:posterior_small_ball} analogous to \cite[Lemma 3, Sec 4.3]{van2011information}. Note that our Gaussian measure is centred around $\mu_D$, hence we define small ball probability in \eqref{eq:covering_relation} w.r.t. to $\mu_D$.
\end{proof}

% \manish{Couple of doubts
% \begin{itemize}
%     \item Since the covering number is with min operator, I think \eqref{eq:covering_relation} holds. But can there be cases where a smaller space has a larger covering number? I am doubtful because ball centres are constrained to lie in the RKHS unit ball. --- ball center can be outside of the RKHS space as well.
%     \item To invoke \cite[Theorem 1.2]{li1999approximation}, do we need equality (or same rates of $\epsilon$) in \cref{eq:covering_relation} or does inequality works? Is it clear that the worst covering number results in the worst $\phi(\epsilon)$ to use iff from \cite[Theorem 1.2]{li1999approximation}? 
%     \begin{itemize}
%         \item $H(U_k, \epsilon)$ for both Matern and squared exponential are actually derived using inequality ($\leq$), so I think our upper bound (inequality) can be used to invoke \cite[Theorem 1.2]{li1999approximation} as well.
%     \end{itemize}
%     \item Can we argue that the inequality in \cref{eq:covering_relation} holds due to constant but the $\mathcal{O}$ or rates are still the same?
% \end{itemize}}


% Note that due to \cref{eq:rkhsnorm_equivalence}, we get $\RKHS = \RKHSdata$. This implies that the covering number in the infinity norm is of the same order. Using \cite[Theorem 1.2, (1.3)]{li1999approximation} this further implies that the small ball probability is also of the same order. 

A formal proof of small ball probability bound with priors is in \cite[sec 4.3]{van2011information}.

%using \cite{li1999approximation,kuelbs1993metric}.



% \manish{Do these small ball probabilities also hold for posterior kernels? In the GP-UCB paper there is a statement that $\RKHSdata = \RKHS$ then which implies the covering number (defined with $\epsilon$ ball infinity norm) should not change and hence also the small ball probability bound.
% %
% \\
% %
% The covering number remains unchanged since the RKHS space is identical. Therefore using \cite{li1999approximation,kuelbs1993metric} we get that the order of SBP is also the same. However, the new SBP is defined for a GP with a conditioned kernel and a zero mean GP $g^i - \mu$, which fits our use case.} 

\manish{The first part of the proof above connects a sample which is epsilon close to the true function. The sample doesn't need to lie in the RKHS space, it is in any space but is $\epsilon$ close to the true sample which lies in the RKHS space---So this does not violate the result of with probability one the sample doesn't lie in the RKHS space.}



\subsection{Extra simulation appendix}

% \manish{What else to show? a 3D plot of $\delta, \epsilon, N$?}


\begin{itemize}
    \item Computation of terminal set
    \item Compute N
\end{itemize}

% 1.1347284419364878

The computed terminal set is too small --  need to start very close or otherwise tightening makes it conservative.

\mypar{Computation of Number of samples} We approximate small ball probability by sampling functions from GP posterior model especially using \ref{step:known_constant_c_D} to get tighter sample complexity. 
% We discretize it finer unless it doesn't change. 
Secondly, we have bounded noise, and we use \cref{coro:bounded_noise_Cd} to estimate $C_D$.

\mypar{Computation of robust PI terminal set}
$\rho$ vs  $B_{\epsilon_c}$ relation
\begin{align*}
    V(x^+) \leq \rho V(x)
    \implies A^\top P A - P\leq (1-\rho)P 
\end{align*}
$(1-\rho)P$ is value decrease (shrinkage). We want contraction in $X_f$ by $\epsilon_c$. Let the boundary of $X_f$ is $x_f$.




$x_f^\top P x_f - (x_f - \epsilon_v)^\top P (x_f - \epsilon_v) = (1-\rho) x_f^\top P x_f$

$1 - (1-\epsilon_c)^2 = (1-\rho^2)$

$\max_{x_f \in \|x\|_P} \min_{\| \epsilon_v \|_P \leq \epsilon_c} (x_f - \epsilon_v)^\top P (x_f - \epsilon_v)$

$ 2 x_f^\top P \epsilon_v -  \epsilon_v^\top P  \epsilon_v = (1-\rho) x_f^\top P x_f$

If $\safeInit{f} = \{ \|x\|_P \leq 1 \}$ and $B_{\epsilon_c} = \{ \|x\|_P \leq \epsilon_c \}$

$\forall x \in \safeInit{f}, \forall \epsilon_v \in B_{\epsilon_c}$ then $f(x) + \epsilon_v \in \safeInit{f}$.

$\| f(x) \|_P \leq \rho \|x\|_P, \rho < 1$

$\| f(x) +\epsilon_v\|_P \leq \| f(x) \|_P + \|\epsilon_v\|_P \leq \rho \|x\|_P + \epsilon_c \leq 1 \implies \epsilon \leq 1-\rho$.


\begin{align*}
        &\|f(x)\|_P^2 = \|x^\top A^\top P A x\|_P^2 \leq L^2 \|x\|_p^2\\
    &\implies A^\top P A \leq L P\\
    &\implies P^{-1/2} A^T P A P^{-1/2} \leq P^{-1/2} L P^1/2 = L^2 * I \\
    &\implies  P^{-1/2} A^T P A P^{-1/2} = P^{-1/2} A^T P^{1/2} P^{1/2} A P^{-1/2} = \Tilde{A}^\top \Tilde{A} \leq L^2\\
    &\implies \| P^{1/2} A P^{-1/2} \|_2 = L 
\end{align*}

\mypar{Computation of tightening to implement in SQP}
subtracting of ellipse from line constraints
% \manish{Can I just subtract the tightening in the omega axis? Technically, this is doable since unknown dynamics are only in the omega dimension.}


% \begin{align*}
%   \!\!\!  \begin{bmatrix}
%         \theta(\ki+1) \\
%         \omega(\ki+1)
%     \end{bmatrix}  \!=\!  \begin{bmatrix}
%         \theta(\ki) + \omega(\ki) \Delta\\
%         \omega(\ki) + (K_1\theta(k) + K_2\omega(k))\Delta
%     \end{bmatrix} \!\! + \!\! \begin{bmatrix}
%         0\\
%         1
%     \end{bmatrix} \!
%     \underbrace{\begin{bmatrix}
%         \frac{-g_a \sin(\theta(\ki)) \Delta}{l} + v\Delta
%     \end{bmatrix}}_{\eqqcolon \dynGP(\state, \coninput)} . 
% \end{align*}


% \begin{align*}
%   \!\!\!\!\!\!  \begin{bmatrix}
%         \theta(\ki+1) \\
%         \omega(\ki+1)
%     \end{bmatrix}  \!=\!  \begin{bmatrix}
%         \theta(\ki) + \omega(\ki) \Delta\\
%         \omega(\ki) + K_2\omega(k)\Delta
%     \end{bmatrix} \!\! + \!\! \begin{bmatrix}
%         0\\
%         1
%     \end{bmatrix} \!
%     \underbrace{\begin{bmatrix}
%         \frac{-g_a \sin(\theta(\ki)) \Delta}{l} + (K_1 \theta(k) + v)\Delta
%     \end{bmatrix}}_{\eqqcolon \dynGP(\state, \coninput)} . 
% \end{align*}


==> literature_amon_edit.tex <==
@article{andersson_casadi_2019,
  title = {{{CasADi}}: A Software Framework for Nonlinear Optimization and Optimal Control},
  shorttitle = {{{CasADi}}},
  author = {Andersson, Joel A. E. and Gillis, Joris and Horn, Greg and Rawlings, James B. and Diehl, Moritz},
  year = {2019},
  journal = {Math. Prog. Comp.},
  volume = {11},
  number = {1},
  doi = {10.1007/s12532-018-0139-4}
}

@article{beckers_prediction_2020,
  title = {Prediction with Gaussian Process Dynamical Models},
  author = {Beckers, Thomas and Hirche, Sandra},
  year = {2020},
  journal = {IEEE Transactions on Automatic Control (submitted)}
}

@article{beckers_prediction_2021,
  title = {Prediction with {{Approximated Gaussian Process Dynamical Models}}},
  author = {Beckers, Thomas and Hirche, Sandra},
  year = {2021},
  journal = {IEEE Transactions on Automatic Control},
  doi = {10.1109/TAC.2021.3131988}
}

@article{berkenkamp_bayesian_2023,
  title = {Bayesian Optimization with Safety Constraints: Safe and Automatic Parameter Tuning in Robotics},
  shorttitle = {Bayesian Optimization with Safety Constraints},
  author = {Berkenkamp, Felix and Krause, Andreas and Schoellig, Angela P.},
  year = {2023},
  journal = {Mach Learn},
  volume = {112},
  number = {10},
  doi = {10.1007/s10994-021-06019-1}
}

@article{bonzanini_fast_2021,
  title = {Fast Approximate Learning-Based Multistage Nonlinear Model Predictive Control Using {{Gaussian}} Processes and Deep Neural Networks},
  author = {Bonzanini, Angelo D. and Paulson, Joel A. and Makrygiorgos, Georgios and Mesbah, Ali},
  year = {2021},
  journal = {Computers \& Chemical Engineering},
  volume = {145},
  doi = {10.1016/j.compchemeng.2020.107174}
}

@article{bonzanini_learning-based_2022,
  title = {Learning-{{Based SMPC}} for {{Reference Tracking Under State-Dependent Uncertainty}}: {{An Application}} to {{Atmospheric Pressure Plasma Jets}} for {{Plasma Medicine}}},
  shorttitle = {Learning-{{Based SMPC}} for {{Reference Tracking Under State-Dependent Uncertainty}}},
  author = {Bonzanini, Angelo D. and Graves, David B. and Mesbah, Ali},
  year = {2022},
  journal = {IEEE Transactions on Control Systems Technology},
  volume = {30},
  number = {2},
  doi = {10.1109/TCST.2021.3069825}
}

@incollection{bradford_hybrid_2021,
  title = {Hybrid {{Gaussian Process Modeling Applied}} to {{Economic Stochastic Model Predictive Control}} of {{Batch Processes}}},
  booktitle = {Recent {{Advances}} in {{Model Predictive Control}}: {{Theory}}, {{Algorithms}}, and {{Applications}}},
  author = {Bradford, E. and Imsland, L. and Reble, M. and {del Rio-Chanona}, E. A.},
  year = {2021},
  publisher = {Springer International Publishing},
  address = {Cham},
  doi = {10.1007/978-3-030-63281-6_8},
  isbn = {978-3-030-63281-6}
}

@inproceedings{bradford_nonlinear_2019,
  title = {Nonlinear Model Predictive Control with Explicit Back-Offs for {{Gaussian}} Process State Space Models},
  booktitle = {2019 {{IEEE}} 58th {{Conference}} on {{Decision}} and {{Control}} ({{CDC}})},
  author = {Bradford, Eric and Imsland, Lars and {del Rio-Chanona}, Ehecatl Antonio},
  year = {2019},
  doi = {10.1109/CDC40024.2019.9029443}
}

@article{bradford_stochastic_2020,
  title = {Stochastic Data-Driven Model Predictive Control Using Gaussian Processes},
  author = {Bradford, Eric and Imsland, Lars and Zhang, Dongda and {del Rio Chanona}, Ehecatl Antonio},
  year = {2020},
  journal = {Computers \& Chemical Engineering},
  volume = {139},
  doi = {10.1016/j.compchemeng.2020.106844}
}

@article{campi_why_2010,
  title = {Why Is {{Resorting}} to {{Fate Wise}}? {{A Critical Look}} at {{Randomized Algorithms}} in {{Systems}} and {{Control}}},
  shorttitle = {Why Is {{Resorting}} to {{Fate Wise}}?},
  author = {Campi, Marco C.},
  year = {2010},
  journal = {European Journal of Control},
  volume = {16},
  number = {5},
  doi = {10.3166/ejc.16.419-430}
}

@article{cao_gaussian_2017,
  title = {Gaussian {{Process Model Predictive Control}} of an {{Unmanned Quadrotor}}},
  author = {Cao, Gang and Lai, Edmund M.-K. and Alam, Fakhrul},
  year = {2017},
  journal = {J Intell Robot Syst},
  volume = {88},
  number = {1},
  doi = {10.1007/s10846-017-0549-y}
}

@inproceedings{capone_localized_2020,
  title = {Localized Active Learning of {{Gaussian}} Process State Space Models},
  booktitle = {Proceedings of the 2nd {{Conference}} on {{Learning}} for {{Dynamics}} and {{Control}}},
  author = {Capone, Alexandre and Noske, Gerrit and Umlauft, Jonas and Beckers, Thomas and Lederer, Armin and Hirche, Sandra},
  year = {2020},
  publisher = {PMLR},
  note = {\url{https://proceedings.mlr.press/v120/capone20a.html}}
}

@article{carron_data-driven_2019,
  title = {Data-{{Driven Model Predictive Control}} for {{Trajectory Tracking With}} a {{Robotic Arm}}},
  author = {Carron, Andrea and Arcari, Elena and Wermelinger, Martin and Hewing, Lukas and Hutter, Marco and Zeilinger, Melanie N.},
  year = {2019},
  journal = {IEEE Robotics and Automation Letters},
  volume = {4},
  number = {4},
  doi = {10.1109/LRA.2019.2929987}
}

@article{conti_gaussian_2009,
  title = {Gaussian Process Emulation of Dynamic Computer Codes},
  author = {Conti, S. and Gosling, J. P. and Oakley, J. E. and O'Hagan, A.},
  year = {2009},
  journal = {Biometrika},
  volume = {96},
  number = {3},
  eprint = {27798855},
  eprinttype = {jstor},
  publisher = {[Oxford University Press, Biometrika Trust]},
  note = {\url{https://www.jstor.org/stable/27798855}}
}

@inproceedings{deisenroth_analytic_2009,
  title = {Analytic Moment-Based {{Gaussian}} Process Filtering},
  booktitle = {Proceedings of the 26th {{Annual International Conference}} on {{Machine Learning}}},
  author = {Deisenroth, Marc Peter and Huber, Marco F. and Hanebeck, Uwe D.},
  year = {2009},
  publisher = {ACM},
  address = {Montreal Quebec Canada},
  doi = {10.1145/1553374.1553403},
  isbn = {978-1-60558-516-1}
}

@phdthesis{diehl_real-time_2001,
  title = {Real-{{Time Optimization}} for {{Large Scale Nonlinear Processes}}},
  author = {Diehl, M.},
  year = {2001},
  school = {University of Heidelberg}
}

@article{diehl_real-time_2005,
  title = {A {{Real-Time Iteration Scheme}} for {{Nonlinear Optimization}} in {{Optimal Feedback Control}}},
  author = {Diehl, Moritz and Bock, Hans Georg and Schl{\"o}der, Johannes P.},
  year = {2005},
  journal = {SIAM J. Control Optim.},
  volume = {43},
  number = {5},
  doi = {10.1137/S0363012902400713}
}

@book{fasshauer_kernel-based_2015,
  title = {Kernel-Based Approximation Methods Using {{MATLAB}}},
  author = {Fasshauer, Gregory and McCourt, Michael},
  year = {2015},
  eprint = {https://www.worldscientific.com/doi/pdf/10.1142/9335},
  publisher = {WORLD SCIENTIFIC},
  doi = {10.1142/9335}
}

@inproceedings{gardner_gpytorch_2018,
  title = {{{GPyTorch}}: {{Blackbox Matrix-Matrix Gaussian Process Inference}} with {{GPU Acceleration}}},
  shorttitle = {{{GPyTorch}}},
  booktitle = {Advances in {{Neural Information Processing Systems}}},
  author = {Gardner, Jacob and Pleiss, Geoff and Weinberger, Kilian Q and Bindel, David and Wilson, Andrew G},
  year = {2018},
  volume = {31},
  publisher = {Curran Associates, Inc.}
}

@techreport{girard_gaussian_2002,
  type = {Technical {{Report}}},
  title = {Gaussian {{Process}} Priors with {{Uncertain Inputs}}: {{Multiple-Step-Ahead Prediction}}},
  author = {Girard, Agathe and Rasmussen, Carl Edward and {Murray-Smith}, Roderick},
  year = {2002},
  number = {TR-2002-119},
  institution = {Department of Computing Science, University of Glasgow}
}

@inproceedings{girard_gaussian_2002-1,
  title = {Gaussian {{Process Priors}} with {{Uncertain Inputs Application}} to {{Multiple-Step Ahead Time Series Forecasting}}},
  booktitle = {Advances in {{Neural Information Processing Systems}}},
  author = {Girard, Agathe and Rasmussen, Carl and Candela, Joaquin Qui{\~n}onero and {Murray-Smith}, Roderick},
  year = {2002},
  volume = {15},
  publisher = {MIT Press}
}

@article{gros_linear_2020,
  title = {From Linear to Nonlinear {{MPC}}: Bridging the Gap via the Real-Time Iteration},
  shorttitle = {From Linear to Nonlinear {{MPC}}},
  author = {Gros, S{\'e}bastien and Zanon, Mario and Quirynen, Rien and Bemporad, Alberto and Diehl, Moritz},
  year = {2020},
  journal = {International Journal of Control},
  volume = {93},
  number = {1},
  doi = {10.1080/00207179.2016.1222553}
}

@article{hachino_multiple_2011,
  title = {Multiple {{Gaussian}} Process Models for Direct Time Series Forecasting},
  author = {Hachino, Tomohiro and Kadirkamanathan, Visakan},
  year = {2011},
  journal = {IEEJ Transactions on Electrical and Electronic Engineering},
  volume = {6},
  number = {3},
  doi = {10.1002/tee.20651}
}

@inproceedings{hachino_time_2007,
  title = {Time {{Series Forecasting Using Multiple Gaussian Process Prior Model}}},
  booktitle = {2007 {{IEEE Symposium}} on {{Computational Intelligence}} and {{Data Mining}}},
  author = {Hachino, Tomohiro and Kadirkamanathan, Visakan},
  year = {2007},
  doi = {10.1109/CIDM.2007.368931}
}

@inproceedings{hardy_multiple-step_2014,
  title = {Multiple-Step Prediction Using a Two Stage {{Gaussian Process}} Model},
  booktitle = {2014 {{American Control Conference}}},
  author = {Hardy, Jason and Havlak, Frank and Campbell, Mark},
  year = {2014},
  doi = {10.1109/ACC.2014.6859020}
}

@article{hewing_cautious_2020,
  title = {Cautious {{Model Predictive Control Using Gaussian Process Regression}}},
  author = {Hewing, Lukas and Kabzan, Juraj and Zeilinger, Melanie N.},
  year = {2020},
  journal = {IEEE Trans Control Syst Technol},
  volume = {28},
  number = {6},
  doi = {10.1109/TCST.2019.2949757}
}

@article{hewing_learning-based_2020,
  title = {Learning-{{Based Model Predictive Control}}: {{Toward Safe Learning}} in {{Control}}},
  shorttitle = {Learning-{{Based Model Predictive Control}}},
  author = {Hewing, Lukas and Wabersich, Kim P. and Menner, Marcel and Zeilinger, Melanie N.},
  year = {2020},
  journal = {Annu. Rev. Control Robot. Auton. Syst.},
  volume = {3},
  number = {1},
  doi = {10.1146/annurev-control-090419-075625}
}

@article{hewing_scenario-based_2020,
  title = {Scenario-{{Based Probabilistic Reachable Sets}} for {{Recursively Feasible Stochastic Model Predictive Control}}},
  author = {Hewing, Lukas and Zeilinger, Melanie N.},
  year = {2020},
  journal = {IEEE Control Systems Letters},
  volume = {4},
  number = {2},
  doi = {10.1109/LCSYS.2019.2949194}
}

@inproceedings{hewing_simulation_2020,
  title = {On {{Simulation}} and {{Trajectory Prediction}} with {{Gaussian Process Dynamics}}},
  booktitle = {Proceedings of the 2nd {{Conference}} on {{Learning}} for {{Dynamics}} and {{Control}}},
  author = {Hewing, Lukas and Arcari, Elena and Fr{\"o}hlich, Lukas P. and Zeilinger, Melanie N.},
  year = {2020},
  publisher = {PMLR}
}

@article{hewing_simulation_nodate,
  title = {On {{Simulation}} and {{Trajectory Prediction}} with {{Gaussian Process Dynamics}}},
  author = {Hewing, Lukas and Arcari, Elena and Frohlich, Lukas P and Zeilinger, Melanie N}
}

@article{kabzan_learning-based_2019,
  title = {Learning-{{Based Model Predictive Control}} for {{Autonomous Racing}}},
  author = {Kabzan, Juraj and Hewing, Lukas and Liniger, Alexander and Zeilinger, Melanie N.},
  year = {2019},
  journal = {IEEE Robot. Autom. Lett.},
  volume = {4},
  number = {4},
  doi = {10.1109/LRA.2019.2926677}
}

@inproceedings{koller_learning-based_2018,
  title = {Learning-{{Based Model Predictive Control}} for {{Safe Exploration}}},
  booktitle = {2018 {{IEEE Conference}} on {{Decision}} and {{Control}} ({{CDC}})},
  author = {Koller, Torsten and Berkenkamp, Felix and Turchetta, Matteo and Krause, Andreas},
  year = {2018},
  doi = {10.1109/CDC.2018.8619572}
}

@article{lahr_zero-order_2023-1,
  title = {Zero-Order Optimization for {{Gaussian}} Process-Based Model Predictive Control},
  author = {Lahr, Amon and Zanelli, Andrea and Carron, Andrea and Zeilinger, Melanie N.},
  year = {2023},
  journal = {European Journal of Control},
  volume = {74},
  doi = {10.1016/j.ejcon.2023.100862}
}

@inproceedings{lambert_learning_2021,
  title = {Learning {{Accurate Long-term Dynamics}} for {{Model-based Reinforcement Learning}}},
  booktitle = {2021 60th {{IEEE Conference}} on {{Decision}} and {{Control}} ({{CDC}})},
  author = {Lambert, Nathan and Wilcox, Albert and Zhang, Howard and Pister, Kristofer S. J. and Calandra, Roberto},
  year = {2021},
  doi = {10.1109/CDC45484.2021.9683134}
}

@article{landgraf_probabilistic_2023-1,
  title = {Probabilistic Prediction Methods for Nonlinear Systems with Application to Stochastic Model Predictive Control},
  author = {Landgraf, Daniel and V{\"o}lz, Andreas and Berkel, Felix and Schmidt, Kevin and Specker, Thomas and Graichen, Knut},
  year = {2023},
  journal = {Annual Reviews in Control},
  volume = {56},
  doi = {10.1016/j.arcontrol.2023.100905}
}

@inproceedings{lederer_confidence_2020,
  title = {Confidence {{Regions}} for {{Simulations}} with {{Learned Probabilistic Models}}},
  booktitle = {2020 {{American Control Conference}} ({{ACC}})},
  author = {Lederer, Armin and Hao, Qing and Hirche, Sandra},
  year = {2020},
  doi = {10.23919/ACC45564.2020.9147978}
}

@article{lucia_multi-stage_2013,
  title = {Multi-Stage Nonlinear Model Predictive Control Applied to a Semi-Batch Polymerization Reactor under Uncertainty},
  author = {Lucia, Sergio and Finkler, Tiago and Engell, Sebastian},
  year = {2013},
  journal = {Journal of Process Control},
  volume = {23},
  number = {9},
  doi = {10.1016/j.jprocont.2013.08.008}
}

@inproceedings{maddalena2021kpc,
  title = {{{KPC}}: {{Learning-based}} Model Predictive Control with Deterministic Guarantees},
  booktitle = {Learning for Dynamics and Control},
  author = {Maddalena, Emilio T and Scharnhorst, Paul and Jiang, Yuning and Jones, Colin N},
  year = {2021},
  publisher = {PMLR}
}

@article{maiworm_online_2021,
  title = {Online Learning-based Model Predictive Control with {{Gaussian}} Process Models and Stability Guarantees},
  author = {Maiworm, Michael and Limon, Daniel and Findeisen, Rolf},
  year = {2021},
  journal = {Int J Robust Nonlinear Control},
  doi = {10.1002/rnc.5361}
}

@book{nocedal_numerical_2006,
  title = {Numerical Optimization},
  author = {Nocedal, Jorge and Wright, Stephen J.},
  year = {2006},
  series = {Springer Series in Operation Research and Financial Engineering},
  edition = {Second edition},
  publisher = {Springer},
  address = {New York},
  isbn = {0-387-30303-0}
}

@article{ostafew_robust_2016,
  title = {Robust {{Constrained Learning-based NMPC}} Enabling Reliable Mobile Robot Path Tracking},
  author = {Ostafew, Chris J. and Schoellig, Angela P. and Barfoot, Timothy D.},
  year = {2016},
  journal = {The International Journal of Robotics Research},
  volume = {35},
  number = {13},
  publisher = {SAGE Publications Ltd STM},
  doi = {10.1177/0278364916645661}
}

@inproceedings{pan_prediction_2017,
  title = {Prediction under {{Uncertainty}} in {{Sparse Spectrum Gaussian Processes}} with {{Applications}} to {{Filtering}} and {{Control}}},
  booktitle = {Proceedings of the 34th {{International Conference}} on {{Machine Learning}}},
  author = {Pan, Yunpeng and Yan, Xinyan and Theodorou, Evangelos A. and Boots, Byron},
  year = {2017},
  publisher = {PMLR}
}

@article{paulson_efficient_2019,
  title = {An Efficient Method for Stochastic Optimal Control with Joint Chance Constraints for Nonlinear Systems},
  author = {Paulson, Joel A. and Mesbah, Ali},
  year = {2019},
  journal = {Int J Robust Nonlinear Control},
  volume = {29},
  number = {15},
  doi = {10.1002/rnc.3999}
}

@article{paulson_nonlinear_2018,
  title = {Nonlinear {{Model Predictive Control}} with {{Explicit Backoffs}} for {{Stochastic Systems}} under {{Arbitrary Uncertainty}}},
  author = {Paulson, Joel A. and Mesbah, Ali},
  year = {2018},
  journal = {IFAC-PapersOnLine},
  volume = {51},
  number = {20},
  doi = {10.1016/j.ifacol.2018.11.036}
}

@inproceedings{pfefferkorn_exact_2022,
  title = {Exact {{Multiple-Step Predictions}} in {{Gaussian Process-based Model Predictive Control}}: {{Observations}}, {{Possibilities}}, and {{Challenges}}},
  shorttitle = {Exact {{Multiple-Step Predictions}} in {{Gaussian Process-based Model Predictive Control}}},
  booktitle = {2022 {{American Control Conference}} ({{ACC}})},
  author = {Pfefferkorn, Maik and Maiworm, Michael and Findeisen, Rolf},
  year = {2022},
  doi = {10.23919/ACC53348.2022.9867259}
}

@inproceedings{quinonero-candela_propagation_2003,
  title = {Propagation of Uncertainty in {{Bayesian}} Kernel Models - Application to Multiple-Step Ahead Forecasting},
  booktitle = {2003 {{IEEE International Conference}} on {{Acoustics}}, {{Speech}}, and {{Signal Processing}}, 2003. {{Proceedings}}. ({{ICASSP}} '03).},
  author = {{Quinonero-Candela}, Joaquin and Girard, A. and Larsen, J. and Rasmussen, C.E.},
  year = {2003},
  volume = {2},
  publisher = {IEEE},
  address = {Hong Kong, China},
  doi = {10.1109/ICASSP.2003.1202463},
  isbn = {978-0-7803-7663-2}
}

@article{quirynen_uncertainty_2021,
  title = {Uncertainty {{Propagation}} by {{Linear Regression Kalman Filters}} for {{Stochastic NMPC}}},
  author = {Quirynen, Rien and Berntorp, Karl},
  year = {2021},
  journal = {IFAC-PapersOnLine},
  volume = {54},
  number = {6},
  doi = {10.1016/j.ifacol.2021.08.527}
}

@book{rasmussen_gaussian_2006,
  title = {Gaussian Processes for Machine Learning},
  author = {Rasmussen, Carl Edward and Williams, Christopher K. I.},
  year = {2006},
  series = {Adaptive Computation and Machine Learning},
  publisher = {MIT Press},
  address = {Cambridge, Massachusetts},
  isbn = {978-0-262-18253-9},
  lccn = {QA274.4 .R37 2006},
  annotation = {OCLC: ocm61285753}
}

@inproceedings{rohr_probabilistic_2021,
  title = {Probabilistic Robust Linear Quadratic Regulators with {{Gaussian}} Processes},
  booktitle = {Proceedings of the 3rd {{Conference}} on {{Learning}} for {{Dynamics}} and {{Control}}},
  author = {von Rohr, Alexander and {Neumann-Brosig}, Matthias and Trimpe, Sebastian},
  year = {2021},
  publisher = {PMLR},
  note = {\url{https://proceedings.mlr.press/v144/rohr21a.html}}
}

@inproceedings{sforni_learning-driven_2021,
  title = {Learning-Driven {{Nonlinear Optimal Control}} via {{Gaussian Process Regression}}},
  booktitle = {2021 60th {{IEEE Conference}} on {{Decision}} and {{Control}} ({{CDC}})},
  author = {Sforni, Lorenzo and Notarnicola, Ivano and Notarstefano, Giuseppe},
  year = {2021},
  doi = {10.1109/CDC45484.2021.9683153}
}

@inproceedings{solak_derivative_2002-1,
  title = {Derivative {{Observations}} in {{Gaussian Process Models}} of {{Dynamic Systems}}},
  booktitle = {Advances in {{Neural Information Processing Systems}}},
  author = {Solak, E. and {Murray-smith}, R. and Leithead, W. and Leith, D. and Rasmussen, Carl},
  year = {2002},
  volume = {15},
  publisher = {MIT Press}
}

@article{soloperto_learning-based_2018,
  title = {Learning-{{Based Robust Model Predictive Control}} with {{State-Dependent Uncertainty}}},
  author = {Soloperto, Raffaele and M{\"u}ller, Matthias A. and Trimpe, Sebastian and Allg{\"o}wer, Frank},
  year = {2018},
  journal = {IFAC-PapersOnLine},
  volume = {51},
  number = {20},
  doi = {10.1016/j.ifacol.2018.11.052}
}

@inproceedings{umlauft_scenario-based_2018-1,
  title = {Scenario-Based {{Optimal Control}} for {{Gaussian Process State Space Models}}},
  booktitle = {2018 {{European Control Conference}} ({{ECC}})},
  author = {Umlauft, Jonas and Beckers, Thomas and Hirche, Sandra},
  year = {2018},
  doi = {10.23919/ECC.2018.8550458}
}

@inproceedings{vaskov_friction-adaptive_2022,
  title = {Friction-{{Adaptive Stochastic Predictive Control}} for {{Trajectory Tracking}} of {{Autonomous Vehicles}}},
  booktitle = {2022 {{American Control Conference}} ({{ACC}})},
  author = {Vaskov, Sean and Quirynen, Rien and Menner, Marcel and others},
  year = {2022},
  doi = {10.23919/ACC53348.2022.9867523}
}

@article{verschueren_acadosmodular_2022,
  title = {Acados---a Modular Open-Source Framework for Fast Embedded Optimal Control},
  author = {Verschueren, Robin and Frison, Gianluca and Kouzoupis, Dimitris and Frey, Jonathan and van Duijkeren, Niels and Zanelli, Andrea and Novoselnik, Branimir and Albin, Thivaharan and Quirynen, Rien and Diehl, Moritz},
  year = {2022},
  journal = {Math. Prog. Comp.},
  volume = {14},
  number = {1},
  doi = {10.1007/s12532-021-00208-8}
}

@inproceedings{vinogradska_stability_2016,
  title = {Stability of {{Controllers}} for {{Gaussian Process Forward Models}}},
  booktitle = {Proceedings of {{The}} 33rd {{International Conference}} on {{Machine Learning}}},
  author = {Vinogradska, Julia and Bischoff, Bastian and {Nguyen-Tuong}, Duy and Romer, Anne and Schmidt, Henner and Peters, Jan},
  year = {2016},
  publisher = {PMLR}
}

@inproceedings{wilson_efficiently_2020,
  title = {Efficiently Sampling Functions from {{Gaussian}} Process Posteriors},
  booktitle = {Proceedings of the 37th {{International Conference}} on {{Machine Learning}}},
  author = {Wilson, James and Borovitskiy, Viacheslav and Terenin, Alexander and Mostowsky, Peter and Deisenroth, Marc},
  year = {2020},
  publisher = {PMLR},
  note = {\url{https://proceedings.mlr.press/v119/wilson20a.html}}
}

@inproceedings{zanelli_contraction_2019,
  title = {Contraction {{Estimates}} for {{Abstract Real-Time Algorithms}} for {{NMPC}}},
  booktitle = {2019 {{IEEE}} 58th {{Conference}} on {{Decision}} and {{Control}} ({{CDC}})},
  author = {Zanelli, Andrea and {Tran-Dinh}, Quoc and Diehl, Moritz},
  year = {2019},
  doi = {10.1109/CDC40024.2019.9029719}
}




==> sections/9_Algorithm.tex <==
\section{Sampling-based GP-MPC algorithm}


\begin{remark}
    Random Fourier feature-based
\end{remark}


\subsection{Efficient sampling within SQP framework}


\begin{align*}
    \state^\n_{0|0} &= x(t) ,  \n \in \mathcal{N}_t \\
    \state_{i+1}^\n &= \dynNom(\state^\n_i, \coninput_i) + \gpsubspace \dynGP(\state^\n_i,\coninput_i) \\
    \state^\n_{0|0} &= \X \ominus B_{\epsilon'}
\end{align*}

\manish{Initialization:
\begin{align*}
    x_{0|t}^\n=\lambda x(t)+(1-\lambda) x_{1|t-1}^{\n,\star}, \lambda\in [0,1].
\end{align*}
}


\manish{An argument for less number of iterations}

==> v_line_patch.tex <==
\errorcontextlines\maxdimen

% begin vertical rule patch for algorithmicx (http://tex.stackexchange.com/questions/144840/vertical-loop-block-lines-in-algorithmicx-with-noend-option)
\makeatletter

\newcommand*{\algrule}[1][\algorithmicindent]{\makebox[#1][l]{\hspace*{.5em} \vrule height .75\baselineskip depth .3\baselineskip}}%

\newcount\ALG@printindent@tempcnta
\def\ALG@printindent{%
    \ifnum \theALG@nested>0% is there anything to print
        \ifx\ALG@text\ALG@x@notext% is this an end group without any text?
            % do nothing
            \addvspace{-3pt}% FUDGE for cases where no text is shown, to make the rules line up
        \else
            \unskip
            % draw a rule for each indent level
            \ALG@printindent@tempcnta=1
            \loop
                \algrule[\csname ALG@ind@\the\ALG@printindent@tempcnta\endcsname]%
                \advance \ALG@printindent@tempcnta 1
            \ifnum \ALG@printindent@tempcnta<\numexpr\theALG@nested+1\relax% can't do <=, so add one to RHS and use < instead
            \repeat
        \fi
    \fi
    }%
\usepackage{etoolbox}
% the following line injects our new indent handling code in place of the default spacing
\patchcmd{\ALG@doentity}{\noindent\hskip\ALG@tlm}{\ALG@printindent}{}{\errmessage{failed to patch}}
\makeatother
% end vertical rule patch for algorithmicx
